Characterizing the head of the degree distributions of growing networks

The analysis in this paper helps to explain the formation of growing networks with degree distributions that follow extended exponential or power-law tails. We present a generic model in which edge dynamics are driven by a continuous attachment of new nodes and a mixed attachment mechanism that triggers random or preferential attachment. Furthermore, reciprocal edges to newly added nodes are established according to a response mechanism. The proposed framework extends previous mixed attachment models by allowing the number of new edges to vary according to various discrete probability distributions, including Poisson, Binomial, Zeta, and Log-Series. We derive analytical expressions for the limit in-degree distribution that results from the mixed attachment and response mechanisms. Moreover, we describe the evolution of the dynamics of the cumulative in-degree distribution. Simulation results illustrate how the number of new edges and the process of reciprocity significantly impact the head of the degree distribution.

==> effects.tex <==
\section{In-degree Distribution and Formation Mechanisms}\label{section4}
This section showcases the effects of non-constant junction and reciprocal response over the behavior of the in-degree distribution.

In order to investigate the effects, we consider the following mechanisms:
%
\begin{description}
\item[M$1^\prime$] \textit{Constant Junction}: At each time $t$, a new node is added to $V_t$ and connects to a fixed number $a$ of target nodes.
\item[M$3^\prime$] \textit{Constant Reciprocity}: As a response to the attachment of a new node, a fixed number $r$ of the selected nodes establishes a new edge to the new node.
\end{description}
%
\subsection{Non-constant Junction Effects}
According to \cref{theorem3.1,lemma3.1}, the number of new connections impacts the behavior of distribution $Q$.  Furthermore, by \cref{eq3.11,eq3.12,eq3.13} the final in-degree distribution depends on $Q$. Therefore, the number of nodes with degree $k$ and the number of new connections are directly related. To explain such relation in more detail, we analyze the effect produced by allowing the number of new edges to vary according to various discrete probability distributions including Binomial, Geometric, Negative Binomial, Poisson, Zeta, and Log-Series distributions.

\subsubsection{Binomial Distribution}
Consider the case in which the number of new edges created by new node follows a Binomial distribution with fixed parameter $n$ and parameter $\theta\in\left\{0.01,0.25,0.5,0.75,1\right\}$.

\subsection{Non-constant Edge Growth Effects over Networks with constant Reciprocity}

Consider a network sequence constructed following mechanisms M1 and M2 with parameter $q=1.0$. According to \cref{eq3.9,eq3.10,eq3.11}, $Q$-distribution affects the total in \cref{eq5.1}. However, from a certain value $k_{\mathrm{sat}}$, the $Q$-distribution does not xxxxxxxx on the final in-degree distribution. Moreover, \cref{theorem3.1} shows that $Q$-distribution depends on the distribution of $A$.

\begin{itemize}
    \item $A\sim\mathrm{Binomial(n,\theta)}$.
    
    For $p=0$, \cref{eq3.11} can be written as
    %
    \begin{equation}
        P_\infty(k)=\frac{1}{1 + \E[A]}\sum\limits_{j=0}^{k}Q(j)\left(\frac{\E[A]}{1+\E[A]}\right)^{k-j},\quad k\geq 0.\label{eq5.1}
    \end{equation}
    %
    According to \cref{lemma3.1}, $Q$-distribution follows a $\mathrm{Binomial}(n,\theta)$. Since $Q(k)=0$ for $k\geq n+1$, we have that $k_\mathrm{sat}=n$. Therefore,
    %
    \begin{equation}
        P_\infty(k)=\left\{ \begin{array}{lll}
       \frac{1}{1+\E[A]}\sum\limits_{j=0}^{k}Q(j)\left(\frac{\E[A]}{1+\E[A]}\right)^{k-j}& ,& 1\leq k\leq n.\\\\
        \frac{1}{{1+\E[A]}}\left(\frac{\E[A]}{1+\E[A]}\right)^k \left(\frac{\theta +\E[A]}{\E[A]}\right)^n&,&k\geq n+1.
       \end{array}
        \right.
        \label{eq5.2}
    \end{equation}
    %
\end{itemize}

Now, According to \cref{eq3.13} we get
%
\begin{equation}
       P_\infty(k)=\left\{ \begin{array}{lll}
       Q(0)& ,& k=0.\\\\
       \frac{2}{k(k+1)(k+2)}\sum\limits_{j=1}^{k}j(j+1)Q(j)&,&k\geq 1.
       \end{array}
        \right.
        \label{eq5.3}
\end{equation}
%    
Clearly $Q$-distribution affects the total in the sum in \cref{eq5.2}. However, from a certain value $k_{\mathrm{min}}$, the $Q$-distribution does not contribute significantly to the sum. For instance, if $A\sim\mathrm{Binomial(n,\theta)}$ for $k>1$ we can rewrite \cref{eq5.2} as follows.
%
\begin{equation}
P_\infty(k)=\left\{ \begin{array}{lll}
       \frac{2}{k(k+1)(k+2)}\sum\limits_{j=1}^{n}j(j+1)Q(j)& ,& 1\leq k\leq n.\\\\
       \frac{2n\theta \left(2+(n-1)\theta\right)}{k(k+1)(k+2)}&,&k\geq n+1.
       \end{array}
        \right.
        \label{eq5.4}
\end{equation}
%
According to \cref{eq5.2} for $k\geq n+1$ the in-distribution follows a power-law with slope equals three, whereas for $1\leq k\leq n$... (see Figure )
%
\begin{figure}[!hbt]
    \centering
    \subfloat[][$p=1$]{\includegraphics[width=220pt]{XminBinom1.pdf}}~
    \subfloat[][$p=1$]{\includegraphics[width=220pt]{XminBinom2.pdf}}
    
    \subfloat[][$p=0$]{\includegraphics[width=220pt]{XminBinom.pdf}}

    \caption{Caption}
    \label{fig4}
\end{figure}
%
\subsection{Reciprocity Effect}
For the purpose of analysis, we consider two networks driven by mechanisms M$1^\prime$, M2 and M3. The first network corresponds to a pure random attachment network by considering $p=0$. The second network corresponds to a pure preferential attachment network by considering $p=1$.

For each network, reciprocity impacts the number of nodes with in-degree less than or equal to $a$ (see \cref{fig5a,fig5b}). This indicates that we have fewer small degree nodes than expected for a exponential or power-law distribution. A possible explanation for this might be each edge established due to mechanism M3 follows a Bernoulli trial with parameter $q$, and since the number of new edges is constant, the probability distribution $Q$ follows a Binomial distribution with parameters $a$ and $q$, this means that reciprocity produces nodes with at most degree $n$, affecting only the frequency with which these degrees appear in the network (see \cref{fig5c,fig5d}). For both networks, reciprocity impacts the slope of the in-degree distribution (see \cref{fig5e,fig5f}). 
%
\begin{figure}[!hbt]
    \centering
    \subfloat[][]{\includegraphics[width=220pt]{reciprocity3.pdf}\label{fig5a}}
    \subfloat[][]{\includegraphics[width=220pt]{powerlaw1.pdf}\label{fig5b}}
    
    \subfloat[][]{\includegraphics[width=220pt]{reciprocity1.pdf}\label{fig5c}}~
    \subfloat[][]{\includegraphics[width=220pt]{powerlaw2.pdf}\label{fig5d}}
    
    \subfloat[][]{\includegraphics[width=220pt]{reciprocity2.pdf}\label{fig5e}}~
    \subfloat[][]{\includegraphics[width=220pt]{powerlaw3.pdf}\label{fig5f}}
    \caption{Reciprocity effects over the in-degree distribution.}
    \label{fig5}
\end{figure}

==> out-degree.tex <==
\section{Asymptotic Behavior of the Out-Degree Distribution}\label{section4}
This section characterizes the out-degree distribution of a network generated by the algorithm presented in \cref{section2}, from a given seed network $G_0$. It also presents how the dynamics of the out-degree distribution converges to a stationary distribution.\\

Let $\hat{K}_t$ be a random variable that characterizes the out-degree of a node selected uniformly at random from $G_t$. Moreover, let $\hat{P}_t(k)=\mathbb{P}(\hat{K}_t=k)$ denote the probability that a realization of $\hat{K}_t$ equals $k$. The expression $\hat{F}_t(k) = \mathbb{P}(\hat{K}_t > k) = 1 - \sum_{i\leq k} \hat{P}_t(i)$ denotes the complementary cumulative distribution function. Finally, let $\hat{\mathbb{B}}(k)$ denote the probability that a new node has in-degree $k$.\\

Note that the out-degree of a randomly selected node depends on all mechanisms. However, the out-degree of a new node only depends on the distribution of the random variable $A$, i.e., $\hat{\mathbb{B}}(k)=\mathbb{P}(A=k)$. The following theorem guarantees the convergence of the out-degree probability distribution. 

\begin{theorem}\label{theorem4.1}
If $0\leq p\leq 1$ and $0 < q\leq 1$, 
the $\lim\limits_{t\rightarrow\infty}\hat{P}_t(k)$ exists for all $k\geq 0$.
\end{theorem}
\begin{proof}
As before, we determine a recursive expression for $\hat{P}_t(k)$ for $k \geq 0$.
According to \cref{eq2.1,eq2.2,eq2.3}, for a fixed $p$, the probability that the new node connects to a target node $v$ with out-degree $k$ is
%
\begin{align}
    \hat{\pi}_t(k)=q\left(p\frac{k}{e_{t-1}} + (1-p)\frac{1}{n_{t-1}}\right).\label{eq4.1}
\end{align}
%
According to \cref{eq4.1} for $k > 0$, the expected number of nodes with out-degree $k$ is given by
%
\begin{align}
    \hat{\pi}_t(k)\E[A]n_{t-1}\hat{P}_{t-1}(k) = q\left(\frac{p k n_{t-1}\E[A]}{e_{t-1}}+(1-p)\E[A]\right)\hat{P}_{t-1}(k)\label{eq4.2}
\end{align}
%
Using \cref{eq4.2} the expected number of nodes with no outgoing edges is given by
%
\begin{equation}
n_{t}\hat{P}_{t}(0) = n_{t-1}\hat{P}_{t-1}(0)-\hat{\pi}_t(0)\E[A]n_{t-1}\hat{P}_{t-1}(0)+\hat{\mathbb{B}}(0).
\label{eq4.3}
\end{equation}
%
The first term in \cref{eq4.3} represents the expected number of nodes with no outgoing edges at time $t-1$. The second term corresponds to the expected number of nodes with no outgoing edges that establish a link with the new node at time $t$. Finally, $\hat{\mathbb{B}}(0)$ accounts for the expected new nodes attaching to the network with no outgoing edges. Now, the expected number of nodes with out-degree $k>0$ is given by
%
  \begin{align}
    n_{t}\hat{P}_{t}(k) =&~n_{t-1}\hat{P}_{t-1}(k)-\hat{\pi}_t(k)\E[A]n_{t-1}\hat{P}_{t-1}(k)+\hat{\pi}_t\left(k-1\right)\E[A]n_{t-1}\hat{P}_{t-1}(k-1)+\hat{\mathbb{B}}(k).
    \label{eq4.4}
  \end{align}
%
The first term in \cref{eq4.4} represents the expected number of nodes with out-degree $k$ at time $t-1$. The second term represents the expected number of nodes with out-degree $k$ that establish a link with the new node at time $t-1$. The third term represents the expected number of nodes with out-degree $k-1$ that establish a link with the new node by mechanism M3. Finally, the fourth term represents the probability that the new node has out-degree equal to $k$.\\

The proof that the limit exists, follows by induction over $k$.
\begin{itemize}
\item \textbf{Base Case}. When $k=0$, using \cref{eq4.3}, $\hat{P}_t(0)$ can be expressed using the recurrence
%
  \begin{equation}
    \hat{P}_t(0)=\hat{\alpha}_t \hat{P}_{t-1}(0)+\hat{\beta}_t,\label{eq4.5}
  \end{equation}
%
where $\hat{\alpha}_t=1-n_{t}^{-1}\left(1+\hat{\pi}_t(0)\E[A]n_{t-1}\right)$ and $\beta_t=n_t^{-1}\hat{\mathbb{B}}(0)$. The expression in \cref{eq4.5} is a non-autonomous, first-order difference equation with initial condition $\hat{P}_0(0)\in[0,1]$. By induction over $t$, the solution to \cref{eq4.5} is given by
%
  \begin{equation}
    \hat{P}_t(0)=\prod\limits_{i=1}^{t}\hat{\alpha}_i\hat{P}_0(0)+\sum\limits_{i=1}^{t}\prod\limits_{j=i+1}^{t}\hat{\beta}_i\hat{\alpha}_j.\label{eq4.6}
  \end{equation}
As before, as $t\rightarrow\infty$, the first term in \cref{eq4.6} goes to $0$ and the second term in \cref{eq4.6} is the convergent series
%
\[\sum\limits_{i=1}^{\infty}\prod\limits_{j=i+1}^{\infty}\hat{\beta}_j\hat{\alpha}_i=\frac{\hat{\mathbb{B}}(0)}{1+q\E[A](1-p)}.\]
%
Therefore,
%
\[\lim\limits_{t\rightarrow\infty}\hat{P}_t(0)=\frac{\hat{\mathbb{B}}(0)}{1+q\E[A](1-p)}.\]

\item \textbf{Inductive step.} Let $k>0$ and assume that $\lim\limits_{t\rightarrow\infty}\hat{P}_t(k)$ exists. Using \cref{eq4.1,eq4.4} we have
%
\begin{equation}
\label{eq4.7}
\begin{split}
n_{t}\hat{P}_{t}(k+1) =& \left[n_{t-1}-q\left(\frac{p (k+1) n_{t-1}\E[A]}{e_{t-1}}+(1-p)\E[A]\right)\right]\hat{P}_{t-1}(k+1)\\
&+q\left(\frac{p k n_{t-1}\E[A]}{e_{t-1}}+(1-p)\E[A]\right)\hat{P}_{t-1}(k)+\hat{\mathbb{B}}(k+1).
\end{split}
\end{equation}
%
Using \cref{eq4.7} for a large enough $t$, we get
%
\begin{align*}
\left(\frac{(1+q)+q\left(p(k+1)+m(1-p)\right)}{1+q}\right)\hat{P}_t(k+1) \sim \left(\frac{q\left( pk+m(1-p)\right)}{1+q}\right)\hat{P}_t(k)+\hat{\mathbb{B}}(k+1).
\end{align*}
%
By inductive hypothesis
%
\begin{equation*}
\lim_{t\rightarrow\infty}\hat{P}_t(k+1)=\frac{q\left( pk+m(1-p)\right)}{1+q\left(1+p(k+1)+m(1-p)\right)}\lim_{t\rightarrow\infty}\hat{P}_t(k)+\frac{(1+q)\hat{\mathbb{B}}(k+1)}{1+q\left(1+p(k+1)+m(1-p)\right)}.
\end{equation*}
\end{itemize}
Therefore, $\lim\limits_{t\rightarrow\infty}\hat{P}_t(k)$ exists for all $k\geq 0$.

\end{proof}

Let $\hat{P}(k)=\lim\limits_{t\rightarrow\infty}\hat{P}_t(k)$. Applying \cref{theorem3.2} for a particular out-degree $k$, we have
%
\begin{equation}
\hat{P}(k)= \left\{ \begin{array}{lll}
             \dfrac{\hat{\mathbb{B}}(0)}{1 + q (1-p)\E[A]} &   ,  & k = 0 \\
             \\ 
             \frac{q\left( p(k-1)+m(1-p)\right)}{1+q\left(1+pk+m(1-p)\right)}\hat{P}(k-1)+\frac{(1+q)\hat{\mathbb{B}}(k)}{1+q\left(1+pk+m(1-p)\right)} &  ,  & k> 0
             \end{array}
   \right.\label{eq4.8}
\end{equation}
%
By induction, it can be shown that the solution of \cref{eq4.8} is given by
\begin{enumerate}
    \item For $p=0$ and $0 < q \leq 1$,
    \begin{equation}
        \hat{P}(k)=\frac{1}{1 + q\E[A]}\sum\limits_{j=0}^{k}\left(\frac{q\E[A]}{1+q\E[A]}\right)^{k-j}\hat{\mathbb{B}}(j),\quad k\geq 0.
        \label{eq4.9}
    \end{equation}
    \item For $0<p\leq 1$ and $q=1$,
    \begin{equation}
       \hat{P}(k)=\frac{\Gamma\left(k+\frac{m(1-p)}{p}\right)}{\Gamma\left(k+\frac{2+p+m(1-p)}{p}\right)}\sum_{j=0}^{k}\frac{2\Gamma\left(j+\frac{2+p+m(1-p))}{p}\right)\hat{\mathbb{B}}(j)}{\left(2+2(1-p)\E[A]+pj\right)\Gamma\left(j+\frac{m(1-p)}{p}\right)}.
       \label{eq4.10}
    \end{equation}
    \item For $p=1$ and $q=1$,
    \begin{equation}
       P(k)=\left\{ \begin{array}{lll}
             \hat{\mathbb{B}}(0) & , & k = 0 \\
             \\             \frac{2}{k(k+1)(k+2)}\sum\limits_{j=1}^{k}j(j+1)\mathbb{B}(j)& , & k> 0
             \end{array}
             \right.
        \label{eq4.11}
    \end{equation}
\end{enumerate}
